Autonomous Search of Semantic Objects in Unknown Environments

This paper addresses the problem of enabling a robot to search for a semantic object, i.e., an object with a semantic label, in an unknown and GPS-denied environment. For the robot in the unknown environment to detect and find the target semantic object, it must perform simultaneous localization and mapping (SLAM) at both geometric and semantic levels using its onboard sensors while planning and executing its motion based on the ever-updated SLAM results. In other words, the robot must be able to conduct simultaneous localization, semantic mapping, motion planning, and execution in real-time in the presence of sensing and motion uncertainty. This is an open problem as it combines semantic SLAM based on perception and real-time motion planning and execution under uncertainty. Moreover, the goals of the robot motion change on the fly depending on whether and how the robot can detect the target object. We propose a novel approach to tackle the problem, leveraging semantic SLAM, Bayesian Networks, Markov Decision Process, and Real-Time Dynamic Programming. The results in simulation and real experiments demonstrate the effectiveness and efficiency of our approach.

==> Sections/Preliminar.tex <==
\section{Preliminary}
\subsection{Bayesian Network \cite{pearl1988probabilistic}}
\label{sec:bayesian net}
A Bayesian Network is a directed, acyclic graph (DAG) $G= \langle \mathcal{X} ,E\rangle $ representing multivariate probability distribution. Each node $X_i \in \mathcal{X}$ in the graph represents a random variable. Each edge in the graph represent conditional dependence. Edge $X_i\rightarrow X_j$ suggests $X_j$ has a conditional dependence on $X_i$, and $A$ is a parent node of $B$. Each node is attached with a conditional probability distribution $P(X_i \mid \operatorname{Parents}(X_i))$, where $\operatorname{Parents}(X_i)$ is the set of nodes that are $X_i$'s parents in the graph. The joint probability distribution $P(X_1, X_2, \ldots, X_n)$ is represented in factorized form as follows:
\begin{equation}
    P(X_1, X_2, \ldots, X_n) = \prod_{i=1}^{N}P(X_i \mid \operatorname{Parents}(X_i))
\end{equation}

The Bayesian Network can be used for probabilistic inference. Given exact values for some evidence variables $X_2, X_3,  \ldots, X_k$, the posterior probability distribution for a query variable $X_1$ can be represented as:
\begin{equation}
\begin{split}
      &P(X_1\mid X_2,  \ldots, X_k)  = \alpha P(X_1, X_2,   \ldots, X_k)  \\
       = &\alpha \sum_{X_{k+1}}\ldots \sum_{X_{n}} P(X_1,  \ldots, X_k, X_{k+1}, \ldots, X_n)
\end{split}
\end{equation}

We are motivated by the real-world problem of searching an unknown indoor environment for some target object in search and rescue scenarios. More specifically, a robot agent is initialized at a random starting position and orientation in an unseen environment and asked to find a target object instance $o_T$ of category $c_T$ (`find a towel'). No environment map is available, and the agent can only use its sensory input (an RGB-D camera) to navigate. At the end of the task, the agent should either report that it has identified the target object instance with a confidence level greater than $1-\epsilon$ or it has failed to find the target object instance.}

\textcolor{blue}{
This problem requires real-time planning and execution of the robot's motion to perform the following two necessary tasks concurrently, which are intertwined and mutually facilitating: 
\begin{itemize}
    \item simultaneous localization and mapping (SLAM) at both semantic and geometric levels to facilitate the search of the target object;
    \item real-time planning and execution of search motion towards the target object based on semantic SLAM results or to expand and improve semantic SLAM to find and identify the target object. 
\end{itemize}
Such search motions of the robot present novel challenges to real-time robot motion planning as the robot motion  planner must {\em combine} (1) active semantic SLAM with improved SLAM results, (2) real-time motion planning under sensing and motion uncertainty in the partially observed world represented by ever updated semantic SLAM results, and (3) real-time determination of (intermediate) goals of motion on the fly and based on ever improved semantic knowledge.} 

\textcolor{blue}{
This paper addresses the novel challenges by leveraging the probabilistic representation of semantic SLAM outcomes (that have been constantly improved), Bayesian network \cite{russell2010artificial} representation of semantic knowledge relating the target object to surrounding objects, and Markov decision process (MDP) formulation. It introduces a method for determining intermediate motion planning goals on the fly based on semantic information and a novel, adaptive planner that synergizes the above (1)-(3) with a unified approach. 
}

